Iterative Bregman Projections for Regularized Transportation Problems

This article details a general numerical framework to approximate so-lutions to linear programs related to optimal transport. The general idea is to introduce an entropic regularization of the initial linear program. This regularized problem corresponds to a Kullback-Leibler Bregman di-vergence projection of a vector (representing some initial joint distribu-tion) on the polytope of constraints. We show that for many problems related to optimal transport, the set of linear constraints can be split in an intersection of a few simple constraints, for which the projections can be computed in closed form. This allows us to make use of iterative Bregman projections (when there are only equality constraints) or more generally Bregman-Dykstra iterations (when inequality constraints are in-volved). We illustrate the usefulness of this approach to several variational problems related to optimal transport: barycenters for the optimal trans-port metric, tomographic reconstruction, multi-marginal optimal trans-port and in particular its application to Brenier's relaxed solutions of in-compressible Euler equations, partial un-balanced optimal transport and optimal transport with capacity constraints.

==> sections/sec-dikstra-algo-lifting.tex <==
%% REMOVED %%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Lifting over Product Spaces}


The algorithms defined through iterations~\eqref{eq-iter-dystra} and~\eqref{eq-iter-bregmanproj} are not symmetric with respect to the indexing of the constraints $\{\Cc_n\}$, i.e. if we re-order the constraints, the trajectories $\{\pi_n\}_n$ differ.

A way to obtain symmetric iterations can be achieved by lifting the problem over the product space $\bpi = (\pi^\ell)_{\ell=1}^L \in (\Si_N)^L$ and re-cast~\eqref{proj-inter} as the following projection
\eql{\label{eq-projinter-lifted}
	\min \enscond{
		\KLdivL{\bpi}{\bar\bpi} = \sum_{\ell=1}^L \la_\ell \KLdiv{\pi^\ell}{\bar\pi^\ell}
	}{
		\bpi \in \bCc_1 \cap \bCc_2
	}
}
where we introduced a a set of weights $\la \in \RR_+^L$, normalized so that $\sum_\ell \la_\ell=1$.

It is easy to check that similarly to the KL divergence, $\KL_\la$ is a also a $f$-divergence as defined in~\cite{}.

The lifted constraint sets are defined as
\begin{align*}
	\bCc_1 &= \enscond{ 
		\bpi = (\pi^\ell)_{\ell=1}^L \in (\Si_N)^L
	}{
		\forall \ell, \ell', \; \pi^\ell = \pi^{\ell'}
	} \\
	\bCc_2 &= \enscond{ 
		\bpi = (\pi^\ell)_{\ell=1}^L \in (\Si_N)^L
	}{
		\forall \ell, \; \pi^\ell \in \Cc_\ell
	} .
\end{align*}

The projection on $\bCc_2$ is simple to compute since the constraint is separable
\eq{
	\KLprojL_{\bCc_2}(\bar\bpi)
	= \pa{ 
		\KLproj_{\Cc_\ell}(\bar\pi_\ell)
	}_{\ell=1}^L
}
The projection on the diagonal set $\bCc_1$ is computed as described in the following proposition. 

\begin{prop}
	The projection $(\pi^\ell)_{\ell=1}^L = \KLprojL_{\Cc_1}(\bar\bpi)$ satisfies 
	\eq{
		\foralls \ell=1,\ldots,L, \quad
			\pi^\ell = \prod_{r=1}^L (\pi^r)^{\la_r}
	}
	where product and exponentiation should be understood component wise. 
\end{prop}
\begin{proof}
	TODO.
\end{proof}

It is then possible to use iterations~\eqref{eq-iter-bregmanproj} (when the sets $\Cc_\ell$ are affine) or \eqref{eq-iter-dystra} (for the general case) to solve the projection~\eqref{eq-projinter-lifted}, which defines iterations that differs from the one obtained when applying these algorithm directly to~\eqref{proj-inter}.

==> sections/sec-martingale.tex <==
% !TEX root = ../KL-Projections.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Martingale Transport}
\label{sec-martingale}


We suppose given two vectors $x, y \in (\RR^{+,*})^N$ indicating the support of discrete measures $\mu=\sum_i p_i \de_{x_i}$ and $\nu = \sum_i q_i \de_{y_i}$, and that $\Cc_{x,y} \cap \Pp(p,q) \neq \emptyset$ where
\eq{
	\Cc_{x,y} = \enscond{ \pi \in (\RR^+)^{N \times N} }{ \pi y = p \cdot x }
}
where $p \cdot x = (p_i x_i)_i$. This constraint expresses that $\pi$ is the law of a martingale, i.e. it is the law of a random pair $(X_1,X_2)$  which is a martingale.

The martingale transportation problem reads
\eql{\label{eq-martingale-prbm}
	\min_\pi \enscond{ \dotp{C}{\pi} }{ \pi \in \Pi(p,q) \cap \Cc_{x,y} }.
}

Introducing an auxiliary variable $\phi$ with the constraint $\phi=\pi \diag(y)$, we consider the following regularized formulation
\eql{\label{eq-martingale-prbm-regul}
	\min_{\pi,\phi}  
		\dotp{C}{\pi} + \dotp{C \diag(y)^{-1}}{\phi} - \ga E(\pi) - \ga E(\phi) 
	\qstq
	\choice{
		\pi \in \Pi(p,q), \\
		\phi \ones = p \cdot x, \\ 
		\phi=\pi \diag(y).
	}
} 
One easily show that the unique solution of~\eqref{eq-martingale-prbm-regul} converges to the solution of~\eqref{eq-martingale-prbm} with maximum entropy [TODO] when $\ga \rightarrow 0$.

The problem~\eqref{eq-martingale-prbm-regul} corresponds to the computation of a KL projection over the pair of variable $(\pi,\phi)$ since
\eq{
	\min_{\pi,\phi}  \enscond{ \KLdiv{\pi}{\bar\pi} + \KLdiv{\phi}{\bar\phi} }{
		(\pi,\phi) \in \Cc_1 \cap \Cc_2\cap \Cc_3
	}
}
where we have defined
\eq{
	\foralls (i,j), \quad
	\bar\pi_{i,j} = e^{-C_{i,j}/\ga}
	\qandq
	\bar\phi_{i,j} = e^{-C_{i,j} y_j^{-1}/\ga},
}
and where the constraint sets are
\begin{align*}
	\Cc_1 &= \enscond{ (\pi,\phi) }{ \pi \ones = p \qandq \phi \ones = p \cdot x }, \\
	\Cc_2 &= \enscond{ (\pi,\phi) }{ \transp{\pi} \ones = q \qandq \phi \ones = p \cdot x }, \\
	\Cc_3 &= \enscond{ (\pi,\phi) }{ \phi=\pi \diag(y) }
\end{align*}

The KL projection on $\Cc_1$ and $\Cc_2$ are easily computed by using [TODO].

The KL projection on $\Cc_3$ is computed as detailed in the following proposition.

\begin{prop}
	The projection $(\pi,\phi) = \KLproj_{\Cc_3}(\bar\pi,\bar\phi)$ satisfies
	$\phi_{i,j} = \pi_{i,j}y_j$ and
	\eq{
		\foralls (i,j), \quad 
		\pi_{i,j} = \exp\pa{
			\frac{
				y_j \log(\bar\phi_{i,j}/y_j) + \log(\bar\pi_{i,j})
			}{
				y_j + 1
			}
		}.
	}
\end{prop} 
\begin{proof}
	The projection is computed independently for each index $(i,j)$, and using the constraint $\phi_{i,j} = \pi_{i,j}y_j$, it corresponds to the resolution of
	\eq{
		\min_{\pi_{i,j}}
			E(\pi_{i,j}) = 
			\pi_{i,j}y_j \log\pa{ \frac{\pi_{i,j}y_j}{\bar\phi_{i,j}} } + 
			\pi_{i,j} \log\pa{ \frac{\pi_{i,j}}{\bar\pi_{i,j}} }.	
	}	
	Writing down the first order condition $E'(\pi_{i,j})=0$ and solving this equation leads to the announced expression.
\end{proof}


Test case (taken from Touzi-Labordere p.17), the cost is of the form $c(x,y)=(\ln(y/x))^2$ and the maginals are lognormal i.e. $p$ and $q$ are the law of respectively $e^X$ and $e^Y$ with $X$ following $N(-\sigma_0^2/2, \sigma_0^2)$ and $Y$ following $N(-\sigma_1^2/2, \sigma_1^2)$ with $\sigma_0<\sigma_1$ (Touzi and Labordere take $\sigma_0^2=.04$ and $\sigma_1^2=.32$). Note that if $p$ is the law of $e^X$ with $X$ following $N(m, \sigma^2)$ its has a density on $\RR_+$ explicitely given by
\[p(t)=\frac{1}{ t \sigma \sqrt{2\pi}} \exp(-\frac{(\ln(t)-m)^2}{2\sigma^2}).  \]





